GENADA: efficient generative time series adversarial attack framework

Deep learning models are widely used for time series analysis in domains such as healthcare, finance, energy systems, and environmental monitoring. However, these models remain vulnerable to adversarial attacks, where small input perturbations cause severe degradation in predictive performance. Commonly used gradient-based attacks, iterative first-order methods, are computationally burdensome, as they repeatedly backpropagate through the victim model to compute input gradients during a number of iterative refinement steps. We propose a GENerative ADversarial Attack (GENADA) that learns a generative model to produce deceptive perturbations directly in a single forward pass and a procedure to train it. Variants include single-step and iterative generative attack schemes. The validation considers attacks on several neural models and datasets in the time-series domain, a controlled, low-dimensional setting. Empirically, GENADA achieves comparable attack quality to strong baselines while requiring less time to generate perturbations during inference.

==> chapters/theorem.tex <==
\subsubsection*{Problem Setup}

Let \(x \in \mathbb{R}^d\) be an input and \(y \in \mathcal Y\) its label.
Let \(C:\mathbb{R}^d \to \mathbb{R}^K\) be a fixed classifier and
\(\ell:\mathbb{R}^K \times \mathcal{Y} \to \mathbb{R}\) a loss function.

\[
f_x(\delta) := \ell(C(x+\delta), y),
\qquad \|\delta\|\le \varepsilon .
\]

We consider the maximization problem
\[
    f_x(\delta) \rightarrow \max 
    \quad \text{s.t. } \|\delta\| \leq \epsilon.
\]

\[
\delta_x^\star = \arg\max_{\|\delta\|\le \varepsilon} f_x(\delta).
\]

Let the generator be a parametric mapping
\[
G_\theta : \mathbb{R}^d \to \mathbb{R}^d,
\]
and we train it by \textbf{maximizing} the objective
\[
J(\theta) := \mathbb{E}_{x \sim \mathcal{D}} \, f_x(G_\theta(x)).
\]

The theoretical justification and proof are presented in the Appendix \ref{sec:theor_justification}.

% \subsubsection*{Assumptions}
% The choice of these assumptions is motivated by a balance between mathematical tractability and the typical behavior observed in deep learning and adversarial robust optimization:

% % \begin{itemize}
% %     \item \textbf{A1 ($L$-smoothness):} This is a standard regularity assumption in non-convex optimization. In the context of adversarial attacks (like FGSM or PGD), assuming Lipschitz continuity of the loss gradient w.r.t. the perturbation $\delta$ is standard practice for proving convergence bounds (e.g., in Sinha et al., 2018). While ReLU activations can make the loss non-smooth at specific points, smoothed variants (like GELU or Softplus) or empirical observation of local smoothness under small $\varepsilon$ justify this assumption in practice.
    
% %     \item \textbf{A2 (Uniform approximation capacity):} This assumption relies on the Universal Approximation Theorems for neural networks (Hornik et al., 1989). Since the perturbation space is bounded by $\|\delta\| \le \varepsilon$ and the input domain is typically compact (e.g., images in $[0, 1]^d$), a sufficiently wide or deep generator network $G_\theta$ is theoretically capable of uniformly approximating the optimal perturbation mapping $\delta_x^\star$. Similar expressivity assumptions are routinely used in the analysis of GANs and neural operators.
    
% %     \item \textbf{A3 (Polyak--Łojasiewicz condition):} The PL condition is significantly weaker than strict concavity, as it allows for multiple local maxima and non-convex landscapes, which is exactly the case for neural network objectives $J(\theta)$. Recent deep learning theory literature (e.g., Allen-Zhu et al., 2019; Liu et al., 2022) shows that overparameterized neural networks often satisfy the PL condition locally or globally during gradient descent. Here, it elegantly captures the property that if the gradient of the generator's objective is small ($\varepsilon_{\mathrm{grad}}$), the generator is close to the optimal achievable utility $J(\theta^\star)$.
% % \end{itemize}

% We consider three assumptions:
% \begin{itemize}
% \item[A1] $L$-smoothness of $f_x(\delta)$ with respect to \(\delta\):
% \[
% \forall x, \delta_1, \delta_2: \|\delta_i\|\le\varepsilon 
% \Rightarrow 
% \|\nabla f_x(\delta_1) - \nabla f_x(\delta_2)\|
% \le
% L \|\delta_1-\delta_2\|.
% \]

% This is a standard regularity assumption in non-convex optimization. In the context of adversarial attacks (like FGSM or PGD), assuming Lipschitz continuity of the loss gradient w.r.t. the perturbation $\delta$ is standard practice for proving convergence bounds (e.g., in Sinha et al., 2018). While ReLU activations can make the loss non-smooth at specific points, smoothed variants (like GELU or Softplus) or empirical observation of local smoothness under small $\varepsilon$ justify this assumption in practice.

% \item[A2] Uniform approximation capacity of the generator:
% \[
% \forall \eta>0\; \exists \theta^\star: 
% \sup_{x}
% \|G_{\theta^\star}(x) - \delta_x^\star\|
% \le \eta.
% \]

% This assumption relies on the Universal Approximation Theorems for neural networks (Hornik et al., 1989). Since the perturbation space is bounded by $\|\delta\| \le \varepsilon$ and the input domain is typically compact (e.g., images in $[0, 1]^d$), a sufficiently wide or deep generator network $G_\theta$ is theoretically capable of uniformly approximating the optimal perturbation mapping $\delta_x^\star$. Similar expressivity assumptions are routinely used in the analysis of GANs and neural operators.

% \item[A3] Polyak--Łojasiewicz (PL) condition for $J(\theta)$:
% \[
% \exists \mu_\theta>0: \forall \theta 
% \Rightarrow 
% \frac12 \|\nabla_\theta J(\theta)\|^2
% \ge
% \mu_\theta \big(J(\theta^\star) - J(\theta)\big).
% \]

% The PL condition is significantly weaker than strict concavity, as it allows for multiple local maxima and non-convex landscapes, which is exactly the case for neural network objectives $J(\theta)$. Recent deep learning theory literature (e.g., Allen-Zhu et al., 2019; Liu et al., 2022) shows that overparameterized neural networks often satisfy the PL condition locally or globally during gradient descent. Here, it elegantly captures the property that if the gradient of the generator's objective is small ($\varepsilon_{\mathrm{grad}}$), the generator is close to the optimal achievable utility $J(\theta^\star)$.
% % \end{itemize}

% \end{itemize}


% \subsubsection*{Theorem}

% Now we can formulate theorem, that proofs workability of our method.

% \begin{theorem}
% Suppose the assumptions [A1]-[A3] hold, and let \(\theta_k\) satisfy
% \[
% \|\nabla_\theta J(\theta_k)\| \le \varepsilon_{\mathrm{grad}}.
% \]
% Then
% \[
% \mathbb{E}_{x}
% \big[
% f_x(\delta_x^\star)
% -
% f_x(G_{\theta_k}(x))
% \big]
% \le
% \frac{L}{2}\eta^2
% +
% \frac{\varepsilon_{\mathrm{grad}}^2}{2\mu_\theta}.
% \]
% \end{theorem}

% \begin{proof} \
% \paragraph{I. Approximation error contribution.}

% By the approximation capacity of the generator, for any \(\eta>0\) there exists \(\theta^\star\) such that
% \[
% \|G_{\theta^\star}(x) - \delta_x^\star\| \le \eta
% \quad \forall x.
% \]

% By $L$-smoothness of $f_x$, it admits the quadratic upper bound
% \[
% \forall \delta_1, \delta_2 \Rightarrow 
% f_x(\delta_1)
% \le
% f_x(\delta_2)
% +
% \langle \nabla f_x(\delta_2), \delta_1-\delta_2 \rangle
% +
% \frac{L}{2}\|\delta_1-\delta_2\|^2.
% \]

% Applying this inequality with
% \(\delta_1 = G_{\theta^\star}(x)\) and
% \(\delta_2 = \delta_x^\star\), we obtain
% \[
% f_x(G_{\theta^\star}(x))
% \le
% f_x(\delta_x^\star)
% +
% \langle \nabla f_x(\delta_x^\star),
% G_{\theta^\star}(x) - \delta_x^\star \rangle
% +
% \frac{L}{2}\eta^2.
% \]

% The first-order optimality condition for $\delta_x^\star$ in the constrained maximization problem over the $\varepsilon$-ball yields
% \[
% \forall \delta': \|\delta'\| \leq \epsilon 
% \Rightarrow 
% \langle \nabla f_x(\delta_x^\star),
% \delta' - \delta_x^\star \rangle
% \le 0.
% \]

% Taking $\delta' = G_{\theta^\star}(x)$ gives
% \[
% \langle \nabla f_x(\delta_x^\star),
% G_{\theta^\star}(x) - \delta_x^\star \rangle
% \le 0,
% \]
% and therefore
% \[
% f_x(\delta_x^\star)
% -
% f_x(G_{\theta^\star}(x))
% \le
% \frac{L}{2}\eta^2.
% \]

% Taking expectation over \(x\):
% \[
% J(\theta^\star)
% \ge
% \mathbb{E}_x f_x(\delta_x^\star)
% -
% \frac{L}{2}\eta^2.
% \]

% \paragraph{II. Optimization error contribution.}

% From the PL condition for $J(\theta)$ and \(\|\nabla_\theta J(\theta_k)\|\le\varepsilon_{\mathrm{grad}}\),
% \[
% \frac12 \varepsilon_{\mathrm{grad}}^2
% \ge
% \mu_\theta \big(J(\theta^\star) - J(\theta_k)\big),
% \]
% hence
% \[
% J(\theta^\star) - J(\theta_k)
% \le
% \frac{\varepsilon_{\mathrm{grad}}^2}{2\mu_\theta}.
% \]

% \paragraph{III. Final bound.}

% \[
% \mathbb{E}_x f_x(\delta_x^\star)
% -
% J(\theta_k)
% =
% \big(
% \mathbb{E}_x f_x(\delta_x^\star)
% -
% J(\theta^\star)
% \big)
% +
% \big(
% J(\theta^\star) - J(\theta_k)
% \big).
% \]

% Using the bounds from Steps I and II,
% \[
% \mathbb{E}_x f_x(\delta_x^\star)
% -
% J(\theta_k)
% \le
% \frac{L}{2}\eta^2
% +
% \frac{\varepsilon_{\mathrm{grad}}^2}{2\mu_\theta}.
% \]

% \end{proof}


==> tables/big_table.tex <==

\begin{table*}[t]
\centering
\caption{Fooling rate (FR) for different attacks and target models.}
\label{tab:results_fr}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccccccccc}
\toprule
Attack & Generator & \multicolumn{3}{c}{PowerCons} & \multicolumn{3}{c}{\cellcolor{verylightgray} GunPoint} & \multicolumn{3}{c}{Strawberry} \\
% \cline{3-5} \cline{6-8} \cline{9-11}
 & & LSTM & PatchTST & ResCNN & \cellcolor{verylightgray} LSTM & 
 \cellcolor{verylightgray} PatchTST & 
 \cellcolor{verylightgray} ResCNN & LSTM & PatchTST & ResCNN \\
\midrule
FGSM & --- & \textit{0.361} & 0.382 & 0.382 & 0.533 & 0.876 & 0.064 & \textit{0.824} & 0.629 & 0.227 \\
iFGSM & --- & 0.113 & \textbf{0.674} & \textbf{0.887} & \textbf{0.82} & \textbf{0.969} & \textbf{0.989} & \textbf{0.873} & 0.893 & \textit{0.969} \\
GENADA & LSTM & 0.152 & 0.32 & 0.378 & 0.173 & 0.46 & 0.391 & 0.406 & 0.49 & 0.345 \\
GENADA & PatchTST & 0.185 & 0.389 & 0.456 & 0.522 & 0.718 & 0.638 & 0.641 & 0.562 & 0.365 \\
GENADA & ResidualCNN & 0.126 & 0.372 & 0.406 & 0.469 & 0.324 & 0.542 & 0.087 & 0.627 & 0.468 \\
GENADA & RNNA & 0.143 & 0.133 & 0.383 & 0.618 & 0.244 & 0.353 & 0.368 & 0.453 & 0.365 \\
iGENADA & LSTM & 0.189 & 0.446 & 0.356 & 0.216 & 0.46 & 0.404 & 0.305 & 0.487 & 0.368 \\
iGENADA & PatchTST & \textbf{0.674} & 0.409 & 0.463 & 0.52 & 0.662 & 0.698 & 0.641 & 0.562 & 0.365 \\
iGENADA & RNNA & 0.111 & 0.231 & 0.357 & 0.607 & 0.229 & 0.316 & 0.368 & 0.427 & 0.365 \\
iGENADA & LSTM curriculum  & 0.078 & 0.011 & 0.344 & 0.467 & 0.34 & 0.267 & 0.36 & 0.438 & 0.438 \\
iGENADA & PatchTST curriculum  & 0.1 & 0.572 & \textit{0.744} & \textit{0.773} & \textit{0.907} & 0.773 & 0.757 & 0.9 & 0.438 \\
iGENADA & ResCNN curriculum  & 0.078 & 0.128 & 0.344 & 0.547 & 0.233 & 0.547 & 0.519 & 0.554 & 0.523 \\
\midrule
Distilled & LSTM & 0.005 & 0 & 0.022 & 0.187 & 0.007 & 0.007 & 0.249 & 0.938 & 0.954 \\
Distilled & ResCNN & 0.011 & 0 & 0.033 & 0.12 & 0.027 & 0.087 & 0.114 & 0.005 & 0.06 \\
Distilled & PatchTST & 0.122 & \textit{0.661} & 0.283 & 0.12 & 0.347 & 0.78 & 0.789 & 0.859 & 0.819 \\
Distilled & RNNA & 0.117 & 0.083 & 0.217 & 0.627 & 0.453 & 0.847 & 0.727 & \textbf{0.951} & 0.959 \\
Distilled & S4 & 0.106 & 0.116 & 0.083 & 0.713 & 0.773 & \textit{0.873} & 0.789 & \textit{0.946} & \textbf{0.973} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/distill_tables.tex <==


\begin{table*}[t]
\centering
\caption{Efficiency (EFF) for different attacks and target models.}
\label{tab:attack_results}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{PowerCons} & \multicolumn{3}{c}{GunPoint} & \multicolumn{3}{c}{Strawberry} \\
\cline{2-10}
Target model
& LSTM & PatchTST & ResCNN
& LSTM & PatchTST & ResCNN
& LSTM & PatchTST & ResCNN \\
\midrule

%Unattacked
%& 1 & 1 & 1
%& 1 & 1 & 1
%& 1 & 1 & 1 \\

%FGSM
%& 0.361 & 0.382 & 0.382
%& 0.533 & 0.876 & 0.064
%& 0.824 & 0.629 & 0.227 \\

iFGSM
& 0.176 & 0.782 & 0.707
& 0.930 & 0.961 & 0.948
& 0.902 & 0.882 & 0.958 \\

%GenLSTM
%& 0.152 & 0.320 & 0.378
%& 0.173 & 0.460 & 0.391
%& 0.406 & 0.490 & 0.345 \\

%GenPatchTST
%& 0.185 & 0.389 & 0.456
%& 0.522 & 0.718 & 0.638
%& 0.641 & 0.562 & 0.365 \\

%GenResidualCNN
%& 0.126 & 0.372 & 0.406
%& 0.469 & 0.324 & 0.542
%& 0.087 & 0.627 & 0.468 \\

Distilled LSTM
& 0.065 & 0.010 & 0.119
& 0.305 & 0.197 & 0.095
& 0.339 & 0.989 & 0.989 \\

Distilled ResCNN
& 0.07 & 0.011 & 0.136
& 0.242 & 0.239 & 0.165
& 0.154 & 0.023 & 0.064 \\

Distilled PatchTST
& 0.164 & 0.575 & 0.449
& 0.307 & 0.289 & 0.789
& 0.835 & 0.982 & 0.770 \\

Distilled RNNA
& 0.12 & 0.088 & 0.301
& 0.757 & 0.649 & 0.845
& 0.729 & 0.951 & 0.957 \\

Distilled S4
& 0.141 & 0.113 & 0.207
& 0.912 & 0.922 & 0.923
& 0.830 & 0.967 & 0.962 \\

% GenS4
% & 0.083 & 0.000 & 0.350
% & -- & -- & --
% & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table*}

%\begin{table*}[t]
%\centering
%\caption{Accuracy (ACC) for different attacks and target models.}
%\label{tab:attack_results}
%\small
%\setlength{\tabcolsep}{4pt}
%\begin{tabular}{lccccccccc}
%\toprule
%& \multicolumn{3}{c|}{PowerCons} & \multicolumn{3}{c|}{GunPoint} & \multicolumn{3}{c}{Strawberry} \\
%\cline{2-10}
%Target model
%& LSTM & PatchTST & ResCNN
%& LSTM & PatchTST & ResCNN
%& LSTM & PatchTST & ResCNN \\
%\midrule
%Unattacked
%& 0.939 & 0.989 & 0.894
%& 0.853 & 0.82 & 0.92
%& 0.849 & 0.976 & 0.954 \\

%FGSM
%& 0.361 & 0.382 & 0.382
%& 0.533 & 0.876 & 0.064
%& 0.824 & 0.629 & 0.227 \\

%iFGSM
%& 0.817 & 0.161 & 0.411
%& 0.113 & 0.02 & 0.027
%& 0.051 & 0.062 & 0.022 \\

%GenLSTM
%& 0.152 & 0.320 & 0.378
%& 0.173 & 0.460 & 0.391
%& 0.406 & 0.490 & 0.345 \\

%GenPatchTST
%& 0.185 & 0.389 & 0.456
%& 0.522 & 0.718 & 0.638
%& 0.641 & 0.562 & 0.365 \\

%GenResidualCNN
%& 0.126 & 0.372 & 0.406
%& 0.469 & 0.324 & 0.542
%& 0.087 & 0.627 & 0.468 \\

%Distilled LSTM
%& 0.933 & 0.989 & 0.883
%& 0.760 & 0.82 & 0.913
%& 0.649 & 0.059 & 0.022 \\

%Distilled ResCNN
%& 0.928 & 0.989 & 0.872
%& 0.787 & 0.787 & 0.86
%& 0.822 & 0.970 & 0.922 \\

%Distilled PatchTST
%& 0.827 & 0.339 & 0.611
%& 0.747 & 0.653 & 0.153
%& 0.095 & 0.138 & 0.184 \\

%Distilled RNNA
%& 0.878 & 0.906 & 0.722
%& 0.293 & 0.36 & 0.127
%& 0.184 & 0.051 & 0.049 \\

%Distilled S4
%& 0.856 & 0.872 & 0.811
%& 0.167 & 0.053 & 0.047
%& 0.1 & 0.046 & 0.040 \\

% GenS4
% & 0.083 & 0.000 & 0.350
% & -- & -- & --
% & -- & -- & -- \\
%\bottomrule
%\end{tabular}
%\end{table*}

==> tables/main_table_old.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|cccc|}
\hline
Dataset & Target-model & Attack & Generator architecture & Fooling rate & Effectiveness & Target accuracy & Time \\
\hline
\multirow{PowerCons} & \multirow{LSTM} & Unattacked & - & 0.0000 & 0.1164 & 0.8759 & - \\
 &  & FGSM & - & 0.3611 & 0.4674 & 0.5222 & - \\
 &  & iFGSM & - & \textbf{0.8833} & \textbf{1.0000} & \textbf{0.0000} & - \\
 &  & Genada & LSTM & 0.1518 & 0.1634 & 0.8389 & - \\
 &  & Genada & ResCNN & 0.1256 & 0.1548 & 0.8663 & - \\
 &  & Genada & PatchTST & 0.1852 & 0.2839 & 0.7019 & - \\
 &  & Iterative Genada & LSTM & 0.1889 & 0.1677 & 0.8500 & - \\
 &  & Iterative Genada & ResCNN & 0.4611 & 0.6241 & 0.5111 & - \\
 &  & Iterative Genada & PatchTST & \underline{0.6741} & \underline{0.6704} & \underline{0.2130} & - \\
\cline{2-8}
 & \multirow{ResCNN} & Unattacked & - & 0.0000 & 0.1165 & 0.8759 & - \\
 &  & FGSM & - & - & - & - & - \\
 &  & iFGSM & - & - & - & - & - \\
 &  & Genada & LSTM & 0.3778 & 0.3333 & 0.5000 & - \\
 &  & Genada & ResCNN & 0.4056 & 0.3182 & 0.5333 & - \\
 &  & Genada & PatchTST & \underline{0.4556} & \underline{0.4229} & \underline{0.4056} & - \\
 &  & Iterative Genada & LSTM & 0.3556 & 0.3233 & 0.5222 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & \textbf{0.4630} & \textbf{0.4305} & \textbf{0.3981} & - \\
\cline{2-8}
 & \multirow{PatchTST} & Unattacked & - & 0.0000 & 0.0733 & 0.9204 & - \\
 &  & FGSM & - & 0.3815 & 0.3845 & 0.4500 & - \\
 &  & iFGSM & - & \textbf{0.5111} & \underline{0.5188} & \textbf{0.3204} & - \\
 &  & Genada & LSTM & 0.3202 & \textbf{0.6798} & 0.5482 & - \\
 &  & Genada & ResCNN & 0.3722 & 0.3209 & 0.6167 & - \\
 &  & Genada & PatchTST & 0.3889 & 0.3823 & 0.4500 & - \\
 &  & Iterative Genada & LSTM & \underline{0.4463} & 0.3083 & 0.5574 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.4093 & 0.4037 & \underline{0.4333} & - \\
\hline
\multirow{Strawberry} & \multirow{LSTM} & Unattacked & - & 0.0000 & 0.0967 & 0.8739 & - \\
 &  & FGSM & - & \textbf{0.8243} & 0.8005 & \underline{0.1108} & - \\
 &  & iFGSM & - & \underline{0.7595} & \textbf{0.9423} & \textbf{0.0297} & - \\
 &  & Genada & LSTM & 0.4063 & 0.4590 & 0.5630 & - \\
 &  & Genada & ResCNN & 0.0865 & 0.2847 & 0.5568 & - \\
 &  & Genada & PatchTST & 0.6405 & \underline{0.9350} & 0.3784 & - \\
 &  & Iterative Genada & LSTM & 0.3045 & 0.4081 & 0.5982 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.6405 & \underline{0.9350} & 0.3784 & - \\
\cline{2-8}
 & \multirow{ResCNN} & Unattacked & - & 0.0000 & 0.0680 & 0.9207 & - \\
 &  & FGSM & - & - & - & - & - \\
 &  & iFGSM & - & - & - & - & - \\
 &  & Genada & LSTM & 0.3450 & 0.2167 & 0.6441 & - \\
 &  & Genada & ResCNN & \textbf{0.4676} & \underline{0.2171} & \underline{0.6432} & - \\
 &  & Genada & PatchTST & 0.3649 & \underline{0.2171} & \underline{0.6432} & - \\
 &  & Iterative Genada & LSTM & \underline{0.3684} & \textbf{0.2987} & \textbf{0.6261} & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.3649 & \underline{0.2171} & \underline{0.6432} & - \\
\cline{2-8}
 & \multirow{PatchTST} & Unattacked & - & 0.0000 & 0.0894 & 0.8874 & - \\
 &  & FGSM & - & \underline{0.6288} & 0.5421 & \underline{0.3108} & - \\
 &  & iFGSM & - & \textbf{0.8595} & \underline{0.9267} & \textbf{0.0387} & - \\
 &  & Genada & LSTM & 0.4901 & 0.7362 & 0.4532 & - \\
 &  & Genada & ResCNN & 0.6270 & 0.4340 & 0.3590 & - \\
 &  & Genada & PatchTST & 0.5622 & \textbf{1.0000} & 0.3568 & - \\
 &  & Iterative Genada & LSTM & 0.4874 & 0.7279 & 0.4559 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.5622 & \textbf{1.0000} & 0.3568 & - \\
\hline
\multirow{GunPoint} & \multirow{LSTM} & Unattacked & - & 0.0000 & 0.1560 & 0.8533 & - \\
 &  & FGSM & - & \underline{0.5333} & \underline{0.7664} & \underline{0.3000} & - \\
 &  & iFGSM & - & \textbf{0.7067} & \textbf{0.8182} & \textbf{0.1000} & - \\
 &  & Genada & LSTM & 0.1734 & 0.3597 & 0.6245 & - \\
 &  & Genada & ResCNN & - & - & - & - \\
 &  & Genada & PatchTST & 0.5222 & 0.5314 & 0.3200 & - \\
 &  & Iterative Genada & LSTM & 0.2156 & 0.3871 & 0.5778 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.5200 & 0.5145 & 0.3356 & - \\
\cline{2-8}
 & \multirow{ResCNN} & Unattacked & - & 0.0000 & 0.3689 & 0.9667 & - \\
 &  & FGSM & - & - & - & - & - \\
 &  & iFGSM & - & - & - & - & - \\
 &  & Genada & LSTM & 0.3911 & 0.3875 & 0.6066 & - \\
 &  & Genada & ResCNN & - & - & - & - \\
 &  & Genada & PatchTST & \underline{0.6378} & \textbf{0.5973} & \underline{0.3645} & - \\
 &  & Iterative Genada & LSTM & 0.4044 & 0.5475 & 0.5933 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & \textbf{0.6978} & \underline{0.5722} & \textbf{0.3133} & - \\
\cline{2-8}
 & \multirow{PatchTST} & Unattacked & - & 0.0000 & 0.1086 & 0.8867 & - \\
 &  & FGSM & - & \underline{0.8756} & \underline{0.9782} & \underline{0.0111} & - \\
 &  & iFGSM & - & \textbf{0.8867} & \textbf{1.0000} & \textbf{0.0000} & - \\
 &  & Genada & LSTM & 0.4600 & 0.3393 & 0.4933 & - \\
 &  & Genada & ResCNN & - & - & - & - \\
 &  & Genada & PatchTST & 0.7178 & 0.6590 & 0.2178 & - \\
 &  & Iterative Genada & LSTM & 0.4600 & 0.3393 & 0.4933 & - \\
 &  & Iterative Genada & ResCNN & - & - & - & - \\
 &  & Iterative Genada & PatchTST & 0.6622 & 0.5929 & 0.2555 & - \\
\hline
\end{tabular}
\caption{Post-attack results averaged over 3 random seeds for various target models and datasets. The best result for each metric inside a dataset+target-model block is bold, the second is underlined.}
\label{tab:attack_results}
\end{table}

==> tables/time.tex <==
\begin{table*}[t]
\centering
\caption{Time for different attacks and target models.}
\label{tab:results_time}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
 & \multicolumn{2}{c|}{dataset} & \multicolumn{2}{c|}{GunPoint} & \multicolumn{2}{c|}{PowerCons} & \multicolumn{2}{c}{Strawberry} \\
\cline{2-3} \cline{4-5} \cline{6-7} \cline{8-9}
Target model & target\_model & LSTM & PatchTST & ResidualCNN & LSTM & PatchTST & ResidualCNN & LSTM & PatchTST & ResidualCNN \\
\midrule
attack & gen\_model & n\_steps & -- & -- & -- & -- & -- & -- & -- & -- \\
fgsm\_attack & GenPatchTST & \textbf{1} & \textbf{0.1050} & \textit{0.0846} & \textit{0.0462} & \textbf{0.0996} & \textbf{0.0697} & \textit{0.0820} & \textit{0.2052} & \textbf{0.1214} \\
train\_attack & GenLSTM & \textit{1} & \textit{0.0211} & \textbf{0.0214} & \textbf{0.0123} & \textit{0.0237} & \textit{0.0388} & \textbf{0.0213} & \textbf{0.0670} & \textit{0.0573} \\
\bottomrule
\end{tabular}
\end{table*}
